Efficient Search of First-Order Nash Equilibria in Nonconvex-Concave Smooth Min-Max Problems

We propose an efficient algorithm for finding first-order Nash equilibria in min-max problems of the form $\min_{x \in X}\max_{y\in Y} F(x,y)$, where the objective function is smooth in both variables and concave with respect to $y$; the sets $X$ and $Y$ are convex and "projection-friendly," and $Y$ is compact. Our goal is to find an $(\varepsilon_x,\varepsilon_y)$-first-order Nash equilibrium with respect to a stationarity criterion that is stronger than the commonly used proximal gradient norm. The proposed approach is fairly simple: we perform approximate proximal-point iterations on the primal function, with inexact oracle provided by Nesterov's algorithm run on the regularized function $F(x_t,\cdot)$, $x_t$ being the current primal iterate. The resulting iteration complexity is $O(\varepsilon_x{}^{-2} \varepsilon_y{}^{-1/2})$ up to a logarithmic factor. As a byproduct, the choice $\varepsilon_y = O(\varepsilon_x{}^2)$ allows for the $O(\varepsilon_x{}^{-3})$ complexity of finding an $\varepsilon_x$-stationary point for the standard Moreau envelope of the primal function. Moreover, when the objective is strongly concave with respect to $y$, the complexity estimate for our algorithm improves to $O(\varepsilon_x{}^{-2}{\kappa_y}^{1/2})$ up to a logarithmic factor, where $\kappa_y$ is the condition number appropriately adjusted for coupling. In both scenarios, the complexity estimates are the best known so far, and are only known for the (weaker) proximal gradient norm criterion. Meanwhile, our approach is "user-friendly:" (i) the algorithm is built upon running a variant of Nesterov's accelerated algorithm as subroutine and avoids extragradient steps; (ii) the convergence analysis recycles the well-known results on accelerated methods with inexact oracle. Finally, we extend the approach to non-Euclidean proximal geometries.

==> related-work.tex <==
\section{Related work}
\label{sec:related-work}

We now give a brief overview of the recent stream of works on efficient algorithms for FNE search in nonconvex-concave problems. %A more comprehensive literature overview can be found in~\cite{lin2019gradient}; however, the rate comparison in their Table 1 seems to have inaccuracies. \odima{should I erase this?}

To the best of our knowledge,~\cite{nouiehed2019solving} was the first work providing non-asymptotic convergence rates for FNE search in general nonconvex-concave problems as in~\cref{opt:min-max}, without assuming special structure of the objective function. 
Their approach is to perform gradient descent %~\odima{is that correct?} 
directly on the primal function of the~$O(\ey)$-regularized version of the problem in~\cref{opt:min-max}, exploiting the fact that this function has~$O(\ey^{-1})$-Lipshitz gradient due to Danskin's theorem. The resulting complexity is~$O(\ex^{-2}{\ey}^{-3/2})$ in our notation, the extra~$O(\ey^{-1})$ factor stemming from the poor smoothness of the primal function, which restricts stepsize to be~$O(\ey)$.

Subtler analyses have been provided in~\cite{thekumparampil2019efficient,kong2019accelerated}, and, more recently, in the concurrent work~\cite{lin2020near} of which we became aware upon finalizing this manuscript, and in the work~\cite{zhao2020primal} that appeared shortly after the first version of this manuscript. 
While the underlying idea of solving the intermediate min-max problem ~\cref{eq:minmax-conceptual-updates} is present in all these works, there are considerable differences between them.
First,~\cite{thekumparampil2019efficient,kong2019accelerated} focus on the problem of finding an~$\ex$-stationary point of the Moreau envelope of the primal function, reducing this problem to that of finding~$(\ex,\ey)$-FNE of the associated min-max problem with~$\ey = O(\ex^2)$. As a result, their complexity writes as~$O(\ex^{-3})$ for the Moreau envelope; nonetheless, we expect their results to be adaptable to the FNE search problem with complexity similar to ours. 
More crucially, the algorithms proposed in these works are somewhat less transparent than ours. In particular,~\cite{thekumparampil2019efficient} runs a mirror-prox type subroutine to approximate the proximal point step (while also using an FGM-type subroutine), and none of these works uses the readily available technical results such as~\cite{devolder2014first} on inexact-oracle FGM, and those of~\cite{lin2015universal,paquette2018catalyst} on the FGM-type implementation of the proximal operator.
 In contrast, our work makes use of the available results to obtain the desired iteration complexity, which results in a more direct analysis and a conceptually simpler algorithm.
 
 %Although not directly relevant to this work, in the context of min-max non-convex-concave optimization, let us also mention~\cite{lu2019block} where  min-max optimization problems  are studied that are non-convex in one variable and linear in the other variable. Also in the context of algorithms without using gradient oracle,   a multi-block  algorithm for non-convex-concave min-max problems was proposed in~\cite{lu2019hybrid} which uses a tight upper-bound of the function instead of using the gradient oracle. In addition, the recent works~\cite{liu2019min, wang2020zeroth}  propose zeroth-order methods for non-convex-concave min-max optimization problems where only use function evaluations.
 
 
% This critique does not apply to the competing work~\cite{lin2020near}, which establishes a rate similar to the one reported in~\cref{th:upper-bound}, for the algorithm closely resembling ours. 
 %Finally, the main focus of~\cite{thekumparampil2019efficient,kong2019accelerated,lin2020near} is on the convex-concave scenario, and the non-convex concave one is considered as a special case; this contributed to somewhat contrived algorithms, except in the case of~\cite{lin2020near}. 
 
%Although not directly relevant to our problem of interest, let us also mention the recent advances in the problem of searching for stationary points in nonconvex minimization problems with a stochastic oracle~\cite{allen2018make,carmon2018accelerated,drori2019complexity,foster2019complexity}, as well as the recent work~\cite{jin2019local} that focuses on the FNE search in the challenging nonconvex-nonconcave scenario with access to a max-oracle.
